Gold Standard Pairs Trading Rules: Are They Valid?

Pairs trading is a strategy based on exploiting mean reversion in prices of securities. It has been shown to generate significant excess returns, but its profitability has dropped significantly in recent periods. We employ the most common distance and cointegration methods on US equities from 1990 to 2020 including the Covid-19 crisis. The strategy overall fails to outperform the market benchmark even with hyperparameter tuning, but it performs very strongly during bear markets. Furthermore, we demonstrate that market factors have a strong relationship with the optimal parametrization for the strategy, and adjustments are appropriate for modern market conditions.

==> tables/adaptive_best.tex <==
\begin{tabular}{lllllllllllllll}
\toprule
            &           & \multicolumn{2}{l}{1990-2000} & \multicolumn{2}{l}{2000-2002} & \multicolumn{2}{l}{2002-2007} & \multicolumn{2}{l}{2007-2009} & \multicolumn{2}{l}{2009-2020} & \multicolumn{2}{l}{2020 (Covid)} &  Average \\
            &           &     Dist. &   Coint. &     Dist. &  Coint. &     Dist. &   Coint. &     Dist. &   Coint. &     Dist. &   Coint. &        Dist. & \multicolumn{2}{l}{Coint.} \\
\midrule
Returns & Monthly profit (adaptive) &   -0.03\% &  -0.05\% &    0.46\% &  0.89\% &    0.10\% &  -0.51\% &    0.64\% &  -0.10\% &   -0.08\% &  -0.05\% &      -0.47\% &  -1.85\% &  -0.09\% \\
            & Monthly profit (best) &    0.88\% &   0.84\% &    0.90\% &  2.04\% &    0.50\% &   0.54\% &    1.18\% &   2.06\% &    0.30\% &   1.00\% &       1.30\% &   1.99\% &   1.13\% \\
            & Monthly profit (finetuned) &    0.38\% &   0.50\% &    0.96\% &  1.45\% &    0.10\% &  -0.09\% &    0.58\% &   0.67\% &   -0.08\% &  -0.12\% &       0.27\% &  -2.04\% &   0.22\% \\
            & Annualized Sharpe (adaptive) &     -0.68 &    -0.47 &      0.78 &     2.0 &      -1.7 &     -4.7 &      0.29 &     -2.1 &      -2.0 &     -2.6 &         -1.3 &     -1.4 &    -1.16 \\
            & Annualized Sharpe (best) &       1.4 &      1.8 &       1.9 &     4.5 &       1.4 &      1.5 &       1.2 &      1.4 &     -0.47 &     0.63 &          5.4 &      4.1 &     2.06 \\
            & Annualized Sharpe (finetuned) &      0.29 &      1.2 &       1.5 &     2.8 &     -0.78 &     -1.7 &     -0.09 &     0.97 &      -1.4 &     -2.3 &         0.15 &     -2.6 &    -0.16 \\
Top params. & \# of pairs &     13.67 &     7.33 &     13.33 &       5 &      7.22 &     6.67 &     28.33 &        5 &     15.33 &        7 &         8.33 &        5 &    10.18 \\
            & Period length mult. &      0.31 &     0.37 &      0.44 &     0.5 &      0.98 &     0.92 &      0.16 &     0.16 &      0.47 &     0.61 &         0.67 &     0.16 &     0.48 \\
            & Confidence &      0.05 &     0.06 &      0.05 &    0.01 &      0.05 &     0.07 &      0.05 &     0.05 &      0.05 &     0.04 &         0.05 &      0.1 &     0.05 \\
            & Threshold &      1.53 &     2.03 &      0.83 &     1.5 &      1.22 &     1.44 &      0.67 &      2.5 &      1.57 &      1.8 &         2.17 &     2.83 &     1.67 \\
\bottomrule
\end{tabular}


==> tables/all_periods_aggregateds.tex <==
\begin{tabular}{lllllll}
\toprule
{} & 1990-2000 & 2000-2002 & 2002-2007 & 2007-2009 & 2009-2020 & 2020 (Covid) \\
{} &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &       Coint. \\
\midrule
Monthly profit            &    0.48\% &    0.72\% &    0.04\% &    1.32\% &   -0.03\% &      -0.99\% \\
Annualized Sharpe         &       1.1 &       1.2 &      -1.6 &       2.2 &      -1.8 &         -1.6 \\
Monthly number of trades  &     0.447 &     0.404 &     0.409 &     0.533 &      0.43 &          0.8 \\
Roundtrip trades          &   51.01\% &   46.55\% &   41.87\% &   54.92\% &   35.37\% &      71.75\% \\
Length of position (days) &      22.3 &      24.5 &      24.8 &      20.9 &      27.4 &         11.8 \\
Pct of winning trades     &   55.41\% &   55.83\% &   55.86\% &   50.45\% &   46.93\% &      62.00\% \\
Max drawdown              &    6.69\% &    9.86\% &    5.59\% &    6.16\% &    4.32\% &      24.48\% \\
Nominated pairs           &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &          5.0 \\
Traded pairs              &   87.02\% &   87.50\% &   90.34\% &   87.27\% &   90.31\% &      90.00\% \\
\bottomrule
\end{tabular}


==> tables/all_periods_aggregatedsyearly.tex <==
\begin{tabular}{lllllllllllllllll}
\toprule
{} & 1990-1992 & 1992-1994 & 1994-1996 & 1996-1998 & 1998-2000 & 2000-2002 & 2002-2004 & 2004-2006 & 2006-2008 & 2008-2010 & 2010-2012 & 2012-2014 & 2014-2016 & 2016-2018 & 2018-2020 & 2020-2020 \\
{} &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. &    Coint. \\
\midrule
Monthly profit            &    0.78\% &    0.06\% &    0.55\% &    0.25\% &    0.87\% &    1.45\% &   -0.57\% &   -0.04\% &    0.35\% &    0.67\% &    0.15\% &   -0.15\% &   -0.46\% &    0.03\% &   -0.17\% &   -2.04\% \\
Annualized Sharpe         &       2.2 &     0.034 &       1.7 &      0.31 &       1.6 &       2.8 &      -2.5 &      -3.1 &      0.32 &      0.97 &     -0.91 &      -2.2 &      -4.4 &      -1.4 &      -2.5 &      -2.6 \\
Monthly number of trades  &     0.458 &     0.411 &     0.417 &     0.383 &     0.417 &     0.411 &     0.356 &     0.411 &     0.444 &     0.456 &     0.444 &     0.411 &      0.35 &     0.433 &      0.39 &     0.644 \\
Roundtrip trades          &   43.96\% &   51.11\% &   67.23\% &   54.31\% &   31.44\% &   53.66\% &   39.44\% &   31.74\% &   44.65\% &   43.26\% &   37.01\% &   32.65\% &   30.91\% &   43.19\% &   32.58\% &   69.22\% \\
Length of position (days) &      23.0 &      19.1 &      18.3 &      19.3 &      30.5 &      20.1 &      26.6 &      22.3 &      24.7 &      26.4 &      22.5 &      28.6 &      31.1 &      22.9 &      27.3 &      11.8 \\
Pct of winning trades     &   58.75\% &   50.83\% &   51.94\% &   49.44\% &   50.42\% &   54.44\% &   55.00\% &   50.83\% &   53.61\% &   55.42\% &   46.94\% &   43.89\% &   34.72\% &   52.50\% &   42.56\% &   42.44\% \\
Max drawdown              &    5.74\% &    5.49\% &    4.41\% &    5.04\% &   11.52\% &    9.16\% &    8.70\% &    4.47\% &    6.08\% &    6.15\% &    4.10\% &    3.69\% &    4.81\% &    3.23\% &    4.60\% &   20.81\% \\
Nominated pairs           &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 &       5.0 \\
Traded pairs              &   92.50\% &   78.33\% &   75.00\% &   76.67\% &   83.33\% &   85.00\% &   85.00\% &   85.00\% &   90.00\% &   85.00\% &   85.00\% &   90.00\% &   78.33\% &   90.00\% &   87.69\% &   73.33\% \\
\bottomrule
\end{tabular}


==> tables/all_periods_aggregatedsyearly_many.tex <==
\begin{tabular}{llllllllllllllllllllllllllllllll}
\toprule
{} & 1990-1991 & 1991-1992 & 1992-1993 & 1993-1994 & 1994-1995 & 1995-1996 & 1996-1997 & 1997-1998 & 1998-1999 & 1999-2000 & 2000-2001 & 2001-2002 & 2002-2003 & 2003-2004 & 2004-2005 & 2005-2006 & 2006-2007 & 2007-2008 & 2008-2009 & 2009-2010 & 2010-2011 & 2011-2012 & 2012-2013 & 2013-2014 & 2014-2015 & 2015-2016 & 2016-2017 & 2017-2018 & 2018-2019 & 2019-2020 & 2020-2020 \\
{} &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. &     Dist. \\
\midrule
Monthly profit            &    0.78\% &    0.51\% &    1.28\% &    1.37\% &    1.10\% &    1.13\% &    1.21\% &    1.26\% &    1.06\% &    1.18\% &    1.43\% &    0.92\% &    1.06\% &    0.62\% &    0.48\% &    0.19\% &    0.95\% &    0.32\% &    1.25\% &    1.28\% &    0.68\% &    0.34\% &    0.60\% &    0.60\% &    0.21\% &    0.37\% &    0.31\% &    0.15\% &    0.10\% &    1.07\% &    1.30\% \\
Annualized Sharpe         &       1.7 &      0.66 &       2.0 &       2.0 &       1.7 &       2.0 &       2.3 &       1.4 &       2.1 &       2.2 &       3.7 &       2.2 &       4.0 &       3.6 &       3.2 &      0.62 &       3.8 &      0.29 &       1.2 &       2.3 &       4.8 &      0.13 &      0.87 &      0.37 &     -0.34 &      0.24 &      0.37 &     -0.35 &      -1.2 &      0.59 &       5.4 \\
Monthly number of trades  &     0.439 &      1.16 &      0.85 &      1.29 &      1.61 &      1.32 &     0.944 &     0.878 &     0.682 &      1.07 &     0.963 &     0.855 &     0.364 &     0.241 &      0.54 &     0.163 &     0.814 &     0.205 &      1.41 &     0.987 &     0.449 &      1.35 &      1.34 &     0.637 &     0.932 &     0.813 &     0.268 &     0.186 &     0.144 &      1.09 &     0.322 \\
Roundtrip trades          &   26.02\% &   48.13\% &   25.28\% &   38.70\% &   45.27\% &   54.30\% &   26.80\% &   21.25\% &   35.49\% &   51.47\% &   49.75\% &   55.54\% &   62.74\% &   55.77\% &   72.52\% &   51.97\% &   40.02\% &   57.57\% &   39.69\% &   42.20\% &   66.59\% &   42.40\% &   39.17\% &   26.13\% &   34.85\% &   46.45\% &   31.76\% &   32.85\% &   34.58\% &   29.04\% &   46.57\% \\
Length of position (days) &      29.6 &      11.2 &       9.0 &       7.0 &       7.1 &      13.4 &       9.0 &       8.1 &      19.7 &      16.9 &      24.1 &      18.6 &      25.5 &      46.4 &      38.6 &      44.1 &      12.9 &      42.8 &       8.4 &      15.7 &      30.6 &       8.1 &       8.3 &      13.0 &      14.0 &      16.9 &      28.1 &      46.0 &      52.8 &       9.7 &      16.4 \\
Pct of winning trades     &   44.94\% &   36.52\% &   35.73\% &   37.67\% &   45.33\% &   40.19\% &   36.94\% &   35.09\% &   43.64\% &   44.50\% &   41.83\% &   45.93\% &   48.73\% &   59.10\% &   49.65\% &   48.06\% &   37.16\% &   38.22\% &   39.56\% &   49.25\% &   27.32\% &   39.47\% &   37.43\% &   30.53\% &   37.95\% &   37.07\% &   37.08\% &   31.26\% &   36.94\% &   30.51\% &   37.84\% \\
Max drawdown              &    7.53\% &    7.17\% &    4.68\% &    4.96\% &    4.79\% &    4.67\% &    4.10\% &    3.87\% &    7.44\% &    8.36\% &    9.26\% &    9.30\% &    7.58\% &    6.28\% &    3.87\% &    4.11\% &    4.23\% &    7.87\% &    4.65\% &    6.47\% &    3.86\% &    2.81\% &    2.67\% &    2.69\% &    2.62\% &    2.83\% &    3.81\% &    2.98\% &    3.39\% &    1.41\% &    4.55\% \\
Nominated pairs           &       5.0 &      33.3 &      11.7 &      16.7 &      28.3 &      6.67 &       5.0 &       5.0 &      16.7 &      18.3 &      8.33 &      30.0 &       5.0 &       5.0 &      6.67 &      6.67 &      11.7 &      21.7 &      30.0 &      40.0 &      20.0 &      26.7 &      15.0 &      10.0 &      10.0 &      6.67 &      6.67 &      20.0 &      6.67 &       5.0 &      8.33 \\
Traded pairs              &   85.00\% &   69.38\% &   62.92\% &   68.61\% &   84.38\% &   71.11\% &   73.33\% &   67.22\% &   69.58\% &   75.56\% &   65.00\% &   71.60\% &   66.67\% &   73.89\% &   65.56\% &   56.67\% &   64.31\% &   53.33\% &   83.68\% &   79.24\% &   39.03\% &   79.58\% &   81.67\% &   63.06\% &   68.75\% &   75.83\% &   56.94\% &   50.35\% &   60.56\% &   76.11\% &   57.33\% \\
\bottomrule
\end{tabular}


==> tables/all_periods_param_avgs.tex <==
\begin{tabular}{lllllll}
\toprule
{} & 1990-2000 & 2000-2002 & 2002-2007 & 2007-2009 & 2009-2020 & 2020 (Covid) \\
\midrule
lag          &         1 &         1 &         1 &         1 &         1 &            1 \\
dist_num     &         5 &         5 &         5 &         5 &         5 &            5 \\
pairs_deltas &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &          0.5 \\
confidence   &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &         0.01 \\
threshold    &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &          2.5 \\
\bottomrule
\end{tabular}


==> tables/all_periods_param_avgsyearly.tex <==
\begin{tabular}{lllllllllllllllll}
\toprule
{} & 1990-1992 & 1992-1994 & 1994-1996 & 1996-1998 & 1998-2000 & 2000-2002 & 2002-2004 & 2004-2006 & 2006-2008 & 2008-2010 & 2010-2012 & 2012-2014 & 2014-2016 & 2016-2018 & 2018-2020 & 2020-2020 \\
\midrule
lag          &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 \\
dist_num     &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 &         5 \\
pairs_deltas &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 &       0.5 \\
confidence   &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 &      0.01 \\
threshold    &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 &       2.5 \\
\bottomrule
\end{tabular}


==> tables/all_periods_param_avgsyearly_many.tex <==
\begin{tabular}{llllllllllllllllllllllllllllllll}
\toprule
{} & 1990-1991 & 1991-1992 & 1992-1993 & 1993-1994 & 1994-1995 & 1995-1996 & 1996-1997 & 1997-1998 & 1998-1999 & 1999-2000 & 2000-2001 & 2001-2002 & 2002-2003 & 2003-2004 & 2004-2005 & 2005-2006 & 2006-2007 & 2007-2008 & 2008-2009 & 2009-2010 & 2010-2011 & 2011-2012 & 2012-2013 & 2013-2014 & 2014-2015 & 2015-2016 & 2016-2017 & 2017-2018 & 2018-2019 & 2019-2020 & 2020-2020 \\
\midrule
lag          &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 &         1 \\
dist_num     &         5 &   33.3333 &   11.6667 &   16.6667 &   28.3333 &   6.66667 &         5 &         5 &   16.6667 &   18.3333 &   8.33333 &        30 &         5 &         5 &   6.66667 &   6.66667 &   11.6667 &   21.6667 &        30 &        40 &        20 &   26.6667 &        15 &        10 &        10 &   6.66667 &   6.66667 &        20 &   6.66667 &         5 &   8.33333 \\
pairs_deltas &       0.5 &  0.273333 &      0.16 &      0.16 &      0.16 &  0.273333 &      0.16 &      0.16 &  0.386667 &      0.44 &      0.66 &  0.553333 &  0.833333 &         1 &      1.16 &      1.22 &  0.273333 &      1.44 &      0.16 &  0.273333 &      1.16 &      0.16 &      0.16 &  0.273333 &  0.273333 &  0.386667 &      0.72 &  0.833333 &   1.05333 &      0.16 &  0.666667 \\
confidence   &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 &      0.05 \\
threshold    &       2.5 &       0.5 &   2.33333 &   1.33333 &  0.833333 &       1.5 &   2.16667 &   2.16667 &       1.5 &  0.666667 &       1.5 &       0.5 &       1.5 &   1.33333 &   1.33333 &   2.16667 &   1.16667 &   1.33333 &         1 &         1 &   2.16667 &  0.833333 &  0.833333 &       2.5 &       1.5 &  0.833333 &         3 &   2.33333 &       2.5 &   1.16667 &   2.16667 \\
\bottomrule
\end{tabular}


==> tables/best_param_avgs.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
{} &  1990-00 &  2000-02 &  2002-07 &  2007-09 &  2009-20 &  Covid &  Total \\
\midrule
\# of pairs         &      10.50 &       9.16 &       6.94 &      16.67 &      11.16 &          6.66 &      15.00 \\
Period length mult. &       0.34 &       0.47 &       0.95 &       0.16 &       0.54 &          0.42 &       0.33 \\
Confidence          &       0.06 &       0.01 &       0.07 &       0.05 &       0.04 &          0.10 &       0.01 \\
Threshold           &       1.78 &       1.16 &       1.33 &       1.58 &       1.68 &          2.50 &       1.58 \\
\bottomrule
\end{tabular}


==> tables/lag_txcost.tex <==
\begin{tabular}{lllrrr}
\toprule
    &   &           & \multicolumn{3}{l}{Transaction cost} \\
    &   &           &            0.000 &  0.003 & 0.005 \\
\midrule
Lag & 0 & # of pairs &             5.00 &   5.83 &  5.83 \\
    &   & Period length mult. &             0.27 &   0.47 &  0.72 \\
    &   & Confidence &             0.08 &   0.06 &  0.05 \\
    &   & Threshold &             1.67 &   2.08 &  2.42 \\
    & 1 & # of pairs &            11.67 &  10.00 &  7.50 \\
    &   & Period length mult. &             0.27 &   0.69 &  0.69 \\
    &   & Confidence &             0.08 &   0.04 &  0.04 \\
    &   & Threshold &             1.42 &   2.25 &  2.58 \\
\bottomrule
\end{tabular}


==> tables/merged_results.tex <==
\begin{tabular}{lllllllllllllllllll}
\toprule
{} & \multicolumn{3}{l}{1990-2000} & \multicolumn{3}{l}{2000-2002} & \multicolumn{3}{l}{2002-2007} & \multicolumn{3}{l}{2007-2009} & \multicolumn{3}{l}{2009-2020} & \multicolumn{3}{l}{2020 (Covid)} \\
{} &     Dist. &   Coint. &   Market &     Dist. &   Coint. &   Market &     Dist. &   Coint. &   Market &     Dist. &   Coint. &   Market &     Dist. &   Coint. &   Market &        Dist. &   Coint. &   Market \\
\midrule
Monthly profit            &    0.16\% &   0.24\% &   0.90\% &    0.25\% &   0.59\% &  -0.83\% &    0.07\% &   0.08\% &   1.15\% &    0.40\% &   0.41\% &  -1.95\% &    0.05\% &   0.14\% &   0.63\% &       0.94\% &  -0.72\% &  -4.79\% \\
Annualized Sharpe         &    -0.068 &     0.48 &     0.64 &       0.3 &      1.8 &     -1.7 &      -1.3 &    -0.89 &      1.1 &       1.0 &     0.72 &     -1.1 &      -1.6 &    -0.64 &     0.94 &          2.2 &     -3.1 &    -0.86 \\
Monthly number of trades  &     0.306 &     0.38 &     None &     0.179 &    0.279 &     None &     0.206 &    0.282 &     None &     0.342 &    0.381 &     None &     0.195 &    0.283 &     None &        0.229 &    0.233 &     None \\
Roundtrip trades          &   51.37\% &  56.73\% &     None &   46.39\% &  57.19\% &     None &   40.81\% &  48.33\% &     None &   53.85\% &  58.30\% &     None &   36.76\% &  46.64\% &     None &      51.62\% &  83.20\% &     None \\
Length of position (days) &      50.5 &     43.2 &     None &      53.8 &     46.7 &     None &      62.2 &     51.6 &     None &      47.9 &     42.5 &     None &      62.1 &     52.2 &     None &         13.4 &     28.6 &     None \\
Pct of winning trades     &   60.49\% &  66.03\% &     None &   48.63\% &  63.93\% &     None &   51.15\% &  61.56\% &     None &   54.78\% &  58.12\% &     None &   49.06\% &  59.83\% &     None &      58.32\% &  52.29\% &     None \\
Max drawdown              &    8.36\% &   9.01\% &  20.57\% &   12.54\% &  12.05\% &  36.50\% &    7.76\% &   8.33\% &  14.63\% &    9.16\% &  10.66\% &  59.01\% &    5.25\% &   6.26\% &  24.22\% &       6.76\% &  11.94\% &  37.58\% \\
Nominated pairs           &      20.0 &     20.0 &     None &      20.0 &     20.0 &     None &      20.0 &     20.0 &     None &      20.0 &     20.0 &     None &      20.0 &     20.0 &     None &         20.0 &     20.0 &     None \\
Traded pairs              &   93.43\% &  97.55\% &     None &   76.13\% &  90.33\% &     None &   83.71\% &  93.45\% &     None &   85.45\% &  86.82\% &     None &   80.28\% &  90.94\% &     None &      58.75\% &  56.67\% &     None \\
\bottomrule
\end{tabular}


==> tables/reshaped_results_simple.tex <==
\begin{tabular}{lllllllll}
\toprule
       &                   & 1990-20 & 2000-02 & 2002-07 & 2007-09 & 2009-20 & Covid & Total \\
\midrule
Dist. & Mo. profit (base) &    0.16\% &    0.25\% &    0.07\% &    0.40\% &    0.05\% &       0.94\% &    0.11\% \\
       & Mo. profit (best) &    0.88\% &    0.90\% &    0.50\% &    1.18\% &    0.30\% &       1.30\% &    0.64\% \\
       & Mo. profit (adaptive) &   -0.03\% &    0.46\% &    0.10\% &    0.64\% &   -0.08\% &      -0.47\% &    0.05\% \\
       & Ann. Sharpe (base) &     -0.07 &       0.3 &      -1.3 &         1 &      -1.6 &          2.2 &     -0.86 \\
       & Ann. Sharpe (best) &       1.4 &       1.9 &       1.4 &       1.2 &     -0.47 &          5.4 &      0.81 \\
       & Ann. Sharpe (adaptive) &     -0.68 &      0.78 &      -1.7 &      0.29 &        -2 &         -1.3 &     -1.16 \\
Coint. & Mo. profit (base) &    0.24\% &    0.59\% &    0.08\% &    0.41\% &    0.14\% &      -0.72\% &    0.18\% \\
       & Mo. profit (best) &    0.84\% &    2.04\% &    0.54\% &    2.06\% &    1.00\% &       1.99\% &    1.03\% \\
       & Mo. profit (adaptive) &   -0.05\% &    0.89\% &   -0.51\% &   -0.10\% &   -0.05\% &      -1.85\% &   -0.11\% \\
       & Ann. Sharpe (base) &      0.48 &       1.8 &     -0.89 &      0.72 &     -0.64 &         -3.1 &     -0.27 \\
       & Ann. Sharpe (best) &       1.8 &       4.5 &       1.5 &       1.4 &      0.63 &          4.1 &      1.57 \\
       & Ann. Sharpe (adaptive) &     -0.47 &         2 &      -4.7 &      -2.1 &      -2.6 &         -1.4 &     -1.96 \\
Market & Mo. profit &    0.90\% &   -0.83\% &    1.15\% &   -1.95\% &    0.63\% &      -4.79\% &    0.47\% \\
       & Ann. Sharpe &      0.64 &      -1.7 &       1.1 &      -1.1 &      0.94 &        -0.86 &      0.38 \\
\bottomrule
\end{tabular}


==> tables/subperiods_summary.tex <==
\begin{tabular}{lllllll}
\toprule
{} &   1990-2000 &   2000-2002 &   2002-2007 &   2007-2009 &   2009-2020 & 2020 (Covid) \\
\midrule
Starting date &  1990-01-01 &  2000-03-01 &  2002-10-01 &  2007-08-01 &  2009-06-01 &   2020-02-20 \\
Ending date   &  2000-03-01 &  2002-10-01 &  2007-08-01 &  2009-06-01 &  2020-02-20 &   2020-06-01 \\
Tx. cost      &      0.0035 &       0.003 &       0.003 &       0.003 &      0.0026 &       0.0026 \\
Short cost    &        0.6% &        0.6% &        0.6% &        0.6% &        0.6% &         0.6% \\
\bottomrule
\end{tabular}

